SpartQA: : A Textual Question Answering Benchmark for Spatial Reasoning

This paper proposes a question-answering (QA) benchmark for spatial reasoning on natural language text which contains more realistic spatial phenomena not covered by prior work and is challenging for state-of-the-art language models (LM). We propose a distant supervision method to improve on this task. Specifically, we design grammar and reasoning rules to automatically generate a spatial description of visual scenes and corresponding QA pairs. Experiments show that further pretraining LMs on these automatically generated data significantly improves LMs' capability on spatial understanding, which in turn helps to better solve two external datasets, bAbI, and boolQ. We hope that this work can foster investigations into more sophisticated models for spatial reasoning over text.

==> experiment.tex <==
%!TEX root=naacl2021.tex
\section{Experiments}
\label{sec:Experiments}
% \subsection{Setup}
% \label{Sec:Setup}

\begin{table*}[t]
    \centering
    \resizebox{0.75\linewidth}{!}{%
      \begin{tabular}{|l|l|c|c|c|c|c|}
        \hline
        \#&Model  & FB  & FR & CO & YN & Avg*\\ %\cline{3-14} 
        \hline
        1&Majority baseline       
             & 28.84 &24.52 & 40.18 &53.60 & 36.64\\
        \hline
        %  \multirow{3}{*}{EXP 1}
        %   &Seen test    & 27.35 &37.73 & 40.38 &67.85 & 43.32\\ \cline{2-2}
        %   &Unseen test   & 20.5  &32.64 & 39.71 &67.74 & 40.14\\ \cline{2-2}
            2&BERT$_{QA}$        
             & 16.34 &20 & 26.16 &45.36 & 30.17\\
        %  EXP 2 &Human& 87.13&69.38& 44.24&85.68\\\hline
        %   \multirow{3}{*}{EXP 2}
        %   &Seen test    & 26.79 &34.13 & 41.33 &67.91 & 42.54\\ \cline{2-2}
        %   &Unseen test   & 23.2  &29.94 & 40.72 &65.82 & 39.92\\ \cline{2-2}
          3&BERT$_{MLM}$--{\small \auto{}(T)}
            & 21.15 &16.19   & 27.1 &51.54 & 32.90\\
          
        4&BERT$_{MLM}$--{\small \auto{}(T+Q)}         & 19.23 &29.54   & \textbf{32.71} &47.42 & 34.88\\
        %   \multirow{3}{*}{EXP 3}
        %   &Seen test    & \textbf{86.85} &\textbf{85.86} & \textbf{71.47} &\textbf{78.29} & \textbf{80.61}\\ \cline{2-2}
        %   &Unseen test   & \textbf{69.77} &\textbf{74.61} & \textbf{61.18} &\textbf{78.06} & \textbf{70.9}\\ \cline{2-2}
          5&BERT$_{QA}$ + \small \auto& \textbf{62.5} &\textbf{46.66} & \textbf{32.71} &47.42  & 47.25\\\hline
          
          6&Human         & 91.66 &95.23 & 91.66 &90.69  &92.31\\\hline
      \end{tabular}
    }
    \caption{Evaluating BERT on \human{}  by four experiments. 1) BERT$_{QA}$, 2) BERT$_{MLM}$--{\small \auto{}(T)}: fine-tuned BERT on \auto{}'s text as MLM task, 3) BERT$_{MLM}$--{\auto{}(T+Q)}: fine-tuned BERT on \auto{}'s text+questions as MLM task, and 4)BERT$_{QA}$--{\small \auto{}}:  fine-tuned BERT on \auto{} as QA task. All models are fine-tuned on \human{} training samples. Avg*: This column shows the weighted average result on all four tasks. All numbers are the accuracy of the models' performance.}
    \label{tab:experiments}
\end{table*} 

\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|l|ccc|ccc|ccc|ccc|}
        \hline
        \multirow{2}{*}{\#}&
        \multirow{2}{*}{Models} & \multicolumn{3}{c}{FB}  & \multicolumn{3}{c}{FR} & \multicolumn{3}{c}{CO} & \multicolumn{3}{c|}{YN}\\ \cline{3-14}
         &&Seen& Unseen& Human*&Seen& Unseen& Human*&Seen& Unseen& Human*&Seen& Unseen& Human*\\ \hline
        %   &&&&&&&&&&&&&\\
          1&Majority &48.70&48.70 & 28.84& 40.81& 40.81 & 24.52& 20.59 &20.38 & 40.18 &49.94 &49.91& \textbf{53.60}\\ 
          \hline
        %   2&BERT_{QA}&  & 13.51& 16.34&&& 20&&& 26.16&&& 45.36&30.17\\
        %   &&&&&&&&&&&&&&\\
        %   BERT + auto-spartQA & - & -& 21.15&-&-& 16.19&-&-& 27.1&-&-& 51.54\\
        %   \multicolumn{1}{|r|}{text_{MLM}}&&&&&&&&&&&&\\
        %   3&BERT_{MLM}&  && &&& 16.19&&& 27.1&&& 51.54&32.90\\
        %   &\small \auto{}(T) &&&&&&&&&&&&&\\
        %   4&BERT_{MLM}&  & & 19.23&&& 29.54&&& 32.71&&& 47.42&34.88\\
        %   &\small \auto{}(T+Q) &&&&&&&&&&&&&\\
        %   BERT + auto-spartQA & - & -& 19.23&-&-& 29.54&-&-& 32.71&-&-& 47.42\\
        %   \multicolumn{1}{|r|}{text+question_{MLM}}&&&&&&&&&&&&\\
        %   BERT^{S}_{QA}& - & -& 62.5&-&-& 46.66&-&-& 32.71&-&-& 47.42\\
        %   &&&&&&&&&&&&\\
        %   BERT +  & - & -& 62.5&-&-& 46.66&-&-& 32.71&-&-& 47.42\\
        %   \multicolumn{1}{|r|}{auto-spartQA_{(QA)}}&&&&&&&&&&&&\\
          
          
         2&BERT & 87.13 & 69.38& 62.5&85.68&73.71& 46.66&71.44&61.09& 32.71&78.29&76.81& 47.42\\ 
        %   &\small \auto{}&&&&&&&&&&&&\\
         3&ALBERT &97.66&83.53& 56.73&91.61 &83.70& 44.76 & 95.20 & 84.55 & 49.53& 79.38&75.05& 41.75\\  
        %  \multicolumn{1}{|r|}{auto-spartQA_{(QA)}}
        %  &\small \auto{}&&&&&&&&&&&&\\
          4&XLNet &\textbf{98.00}&\textbf{84.85} & \textbf{73.07}& \textbf{94.60} &\textbf{91.63}& \textbf{57.14}& \textbf{97.11} &\textbf{90.88} & \textbf{50.46}&\textbf{79.91} &\textbf{78.54}& 39.69\\
        %   \multicolumn{1}{|r|}{auto-spartQA_{(QA)}}
        %   &\small \auto{}&&&&&&&&&&&&\\
          \hline
        %  \multirow{2}{*}{RoBERTa}& 8k& & & & & & & & &\\ \cline{2-2}
        %   &24k & & & & & & & & &\\ \hline
        %  \multirow{2}{*}{LSTM}& 8k& & & & & & & & &\\ \cline{2-2}
        %   &24k & & & & & & & & &\\ \hline
            % &&&&&&&&&&&&\\
          5&Human & \multicolumn{2}{c}{85}&91.66&\multicolumn{2}{c}{90}&95.23&\multicolumn{2}{c}{94.44}&91.66&\multicolumn{2}{c}{90}&90.69\\ \hline
    \end{tabular}
    }
    \caption{Fine-tuning three baseline LMS (BERT, ALBERT, and XLNET) on \auto, and test on three benchmarks, Seen, Unseen and Human~(\human) sets. \textbf{Human*}: For Human result all models are fine-tuned on \human{} training samples. The result of Human on Seen and Unseen test are the same since the changes applied on unseen set does not affect human reasoning. All numbers are reported for the model's accuracy.}
    \label{tab:evaluation}
\end{table*}

\qn{}

We design the following experiments to evaluate whether 
\auto{}
% our automatically generated dataset 
improves the performance of 
modern %baseline
LMs~(i.e., BERT, ALBERT, and XLNet) in spatial reasoning. % over spatial language. 
% All experiments, use the models defined in Section \ref{Sec:Architecture}. We use AdamW~\cite{loshchilov2017decoupled} with $2e-06$ learning rate and Focal Loss~\cite{lin2017focal} with $\gamma = 2$ for training all models.

% We evaluate the performance of pre-trained LMs.
%particularly BERT. 
% The current language models are usually trained on large unlabeled text with generic data domain for two main tasks of Masking Language Model~(MLM) and Next Sentence Prediction~(NSP). In the MLM task, the model must predict some randomly masked tokens, and in the NSP task, it must predict the next sentence based on a given set of previous sentences. 

% \outline{start with spatial ability on LM}\\
% To evaluate the capability of pretrained language models (here BERT) to do spatial reasoning over natural language, we design BERT$_{QA}$ experiment.

% adapt to spatial QA
\paragraph{BERT$_{QA}$}  In this experiment, we use the same architectures described in Sec. \ref{Sec:Architecture} for answering various types of questions. We use the pretrained BERT as its base module. %Then, we fine-tune this proposed model by training on \human{} training samples. 
% \pk{Don't you need to mention what is the fine-tuning data on top of pre-trained BERT?} \rk{Here we just describe the model. Fine-tuning this model on our data comes when we are describing the result of each one of this model.}
% Table \ref{tab:experiments}~(row 2), shows that even after training BERT on \human{}, it cannot perform well on doing spatial understanding and reasoning over them. 

%Hence, we improve this performance by providing external supervision signals.
% \rk{These samples help LM to gain some knowledge about spatial language and to train classifier parameters to be able to do question answering. }

% As pre-trained LM cannot solve our QA task without further fine-tuning, we must fine-tune that on a set of QA examples,~$training_1$. Since collecting a large set of human-generated data to form $training_1$ is time-consuming and expensive, We create a small training set containing 616 samples (around 150 samples for each task) and use them as $training_1$. This small set helps LM to gain some knowledge about spatial language and to train classifier parameters to be able to do question answering.\rk{we can remove the last sentence.}


% \outline{enhance LM}\\
% To enhance BERT on doing spatial reasoning over natural language, we use our automatically generated data, \auto{}. There are two approaches for training BERT on this data, 1) train BERT on MLM task (the same task as it is trained on) or 2) train it on the QA task (which is the same as \human's task).
% spatial expressions instead of term and text

\paragraph{BERT$_{MLM}$--{\small\auto{}(T)}} BERT is pretrained on general-domain texts in BookCorpus~\cite{zhu2015aligning} and Wikipedia articles which do not contain many spatial descriptions.
% \pk{Maybe instead of using LMs just talk about BERT?}\rk{I think here in setup we should talk about all language models in general and then in result (as I have it) we said we use BERT as LM sample} 
For example, in those resources, the word ``right'' is used more frequently to mean ``correct'', or the word ``left'' is used more frequently to mean ``leaving'' rather than their spatial meaning.
%\pk{you can keep this example if you like though this is just an estimate and you do not have any evidence for this claim}\rk{I ckecked this on SQuAD, DROP and HOTPOTQA that used wikipedia article (the same data that LMs pretrained on). should I mentioned this experiment here too?}.
Hence, in this experiment, first, we further pretrain BERT on \auto's stories in the form of the MLM task~(Randomly masking tokens). We use this further pretrained BERT as the base module in the architecture described in Sec. \ref{Sec:Architecture}.%Next, we use the same architecture described in Sec. \ref{Sec:Architecture} to fine-tune the model by training on \human training samples.%~(We call this experiment BERT$_{MLM}$ {\small\auto{}~(T)}).

% Table \ref{tab:experiments}(row 3) indicates that this method does not help and even hurts the performance of BERT in some cases~(FR \qtype).

% Hence, in the first experiment on MLM task \pk{we want let LMs to see some spatial expressions: We train LMs with spatial expressions}\pk{ and see if this can improve its spatial understanding or not.: REMOVE} \pk{To do so: To do the training}, we randomly mask some tokens of each \auto's story and fine-tune the LM on predicting those before further fine-tuning \pk{it: remove} on \human.
\begin{figure}
    \centering
    \includegraphics[width = 0.75\linewidth]{images/mask.pdf}
    \caption{Convert (paragraph, question, answer) to a single text for MLM task. }
    \label{fig:masking}
\end{figure}

\paragraph{BERT$_{MLM}$--{{\small\auto{}(T+Q)}}} BERT$_{MLM}$- {\small\auto{}(T)} model is trained only on the stories of our samples while the the (question,answer) pairs are the main source of supervision for spatial reasoning.
Thus, in this experiment, we add the (question,answer) pair information to the end of the stories using $f(t,q,a)$, where $t$ is the text description~(story), $q$ is the question, and $a$ is the correct answer. We define $f$ as:
\begin{equation}
    f(t,q,a) = t . to\_sentence(q,a)
\end{equation}
where $.$ is the concatenation operator and $to\_sentence(.)$ transforms question, $q$, and its answer, $a$, to a single sentence as shown in Fig.~\ref{fig:masking}.
Then, we further pretrain BERT on the updated stories by masking tokens containing the answer in the form of the MLM task. We use this further pretrained BERT as the base module in the architecture describe in Sec. \ref{Sec:Architecture}. %Then, we fine-tune the model by training on \human{} training samples.
% by casting each (paragraph, question, answer) to a (paragraph + \textit{to\_sentence}(question, answer)) which \textit{to\_sentence} gets aquestion and its answer and transforms them to a single sentence that described the asked relation between objects.
% \pk{it is not clear to me why to-sentence () is used here, any notation should be defined, you can a not expect the reader to decode the notation} 
% where the question and its correct answer are transformed to a single sentence and 
% Finally to the end of the paragraph (image \ref{fig:masking}).
% (We call this experiment ). 


% Comparing rows 3 and 4 of Table \ref{tab:experiments} shows that adding question can improve the average result on all tasks $1.98\%$. Also on FR and CO \qtype{}s, that using BERT$_{MLM}$~( {\small\auto{}~(T)}) decreases~(FR) or marginally improves~(CO) the  BERT$_{QA}$'s accuracy, BERT$_{MLM}$~( {\small\auto{}~(T)}) improves it by 9.54\% on FR and $6.55$ on CO. 

% The result of the fine-tuned BERT with random MLM task on \auto{}~(row 3) indicates that this method does not help and even hurts the performance of BERT in some cases~(FR \qtype). In this experiment, we dismiss questions while questions are the parts which contain the traceable and essential spatial information in the dataset. Therefore, this experiment shows that fine-tuning on additional text without supervision signals from the task is not helpful. On the other hand, fine-tuning BERT on \auto{}'s text+question with selectively masking the answer~(row 3) is helpful while we using the supervision signals in the questions.For instance, the result of FR \qtype{} improves by 9\%.



% \outline{using auto-spartqa}\\
 \paragraph{BERT$_{QA}$--{\small\auto{}}} 
 We use the same setting as BERT$_{QA}$ and train the model further on \auto{} samples.
%  Nevertheless, the problem of the above setting is that it is not capable of including multiple or null answers. Moreover, it is hard to evaluate the answers that  contain multiple tokens~(in CO candidates. e.g. ``big blue circle'' \pk{I assume you have described CO somewhere else and the fact that it has multiple answers? just double check}\rk{here we are mentioning multiple tokens. For example in MLM if the answer is big blue circle, evaluating the model on predicting all these tokens is hard (as we discussed perplexity approach.)}). Thus, to further fine-tune a model we need data in such form that can handle these complexity of target task (here is \human{}.) 
% Thus, we fine-tune baseline LMs on the QA task and evaluate \pk{you say that "we fine-tune by evaluating...?" doesn't sound correct, probably you fine-tune on something and evaluate on something else ... revise this paragraph pls} their performance on spatial reasoning when further fine-tuned on \auto's training set (BERT$_{QA}$ {\small\auto{}}). 
%and then fine-tune the model one more step on $training_1$ to be comparable with other experiments.

% Rows 2 to 5 of the table \ref{tab:experiments} indicate the result~(accuracy) of BERT on four experiments discussed in section \ref{Sec:Setup} on \human{}'s test set. The last column of the table~\ref{tab:experiments} is the average of the results on all \qtype{}s.

% \outline{Start comparing the table's results}
Table \ref{tab:experiments} shows the results of above experiments evaluated on \human{}'s test samples. All these models are fine-tuned~(regardless of their initial training) by training on \human{} training samples.

During our annotation, we found that the description of ``near to '' and ``far from'' varies largely between annotators. Therefore, we ignore these two relations from FR \qtype{} during evaluating \human{} examples to be consistent.

The poor performance of BERT$_{QA}$ shows that pretrained BERT cannot perform well on spatial reasoning based on the available human-generated data. Comparing the average performance of BERT$_{QA}$ to any of the other models shows that further pretraining on our automatically generated data helps BERT-base models to get better spatial reasoning capability. BERT$_{QA}$--{\small \auto{}} achieves the best improvement as it is trained on automatically generated samples using the same target task setting as \human{}.
% \pk{similar samples and setting as the final evaluation task.: automatically generated train using the same target task setting.}

The reason of the improvement on BERT$_{MLM}$--{ {\small\auto{}~(T+Q)}} over BERT$_{MLM}$--{\small\auto{}~(T)} is the first is trained on updated stories which include (question,answer) pairs and the masked tokens are the ones that require spatial reasoning to be predicted while the second is only trained on random masked tokens from the stories.
% \pk{This helped the model to gain a better understanding of the underlying phenomena.: there is NO information in this sentence!} \pk{Maybe this? : This setting gave a more direct supervision to train the LM to do spatial reasoning.}

% Table \ref{tab:experiments}~(row 2), shows that even after training BERT on \human{}, it cannot perform well on doing spatial understanding and reasoning over them. 

% Table \ref{tab:experiments}(row 3) indicates that this method does not help and even hurts the performance of BERT in some cases~(FR \qtype).

% Comparing rows 3 and 4 of Table \ref{tab:experiments} shows that adding question can improve the average result on all tasks $1.98\%$. Also on FR and CO \qtype{}s, that using BERT$_{MLM}$~( {\small\auto{}~(T)}) decreases~(FR) or marginally improves~(CO) the  BERT$_{QA}$'s accuracy, BERT$_{MLM}$~( {\small\auto{}~(T)}) improves it by 9.54\% on FR and $6.55$ on CO. 

% Comparing the result of the BERT$_{QA}$~( table~\ref{tab:experiments} row 2) and BERT$_{QA}$ fine-tuned on \auto{} on different forms of tasks~(QA and MLM -rows 3 to 5) indicates the helpfulness of this data as a distant supervision to understanding spatial language and doing spatial reasoning. Also, the high result of the BERT$_{QA}$~(on {\small\auto{}}) shows that teaching models by answering complex questions that need spatial reasoning over different part of the text and can have multiple-answers, is more effective than other methods. For instance, the result of the FB \qtype{} is improved by $35.07\%$ after using this model.

The only exception is the result of YN \qtype{} on the human test set, which is getting lower results than the the majority baseline~(51.9\%) even after training on \auto{}. Since the human test set is imbalance, we also compute the F1-measure for YN \qtype{} which is shown in Table \ref{tab:f1-YN}. This table shows that after using \dataset{}, models perform better than the majority baseline. The best performance is achieved by BERT fine-tuned on \auto{}'s text as MLM task. This can be due to the complexity of the YN questions (described in Sec. \ref{sec:auto}).
% \pk{have you described why these are complex? If so point to the section that you describe this in here.} 

\begin{table}[h]
    \centering
    \begin{tabular}{|l|c|}
        \hline
        Model & F1-measure \\ \hline
         Majority Baseline& 0.35 \\ \hline
         BERT$_{QA}$& 0.50 \\
         BERT$_{MLM}$--{\small \auto{}(T)} & 0.53\\
         BERT$_{MLM}$--{\small \auto{}(T+Q)} & 0.48\\
         BERT$_{QA}$--{\small \auto{}} & 0.48\\
         \hline
    \end{tabular}
    \caption{Evaluating models on YN \qtype{} with F1-measure.}
    \label{tab:f1-YN}
\end{table}

\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{|l|c|cc|cc|cc|}
        \hline
        \multirow{2}{*}{Models} &  \multicolumn{1}{c}{FB}  & \multicolumn{2}{c}{FR} & \multicolumn{2}{c}{CO} & \multicolumn{2}{c|}{YN}\\ \cline{2-8}
         &Consistency&Consistency&Contrast&Consistency& Contrast&Consistency& Contrast\\ \hline
         \multirow{1}{*}{BERT}   &69.44  &76.13  &42.47  &16.99  &15.58  &48.07   &71.41\\ \hline
         \multirow{1}{*}{AlBERT} &84.77  &82.42  &41.69  &58.42  &62.51  &48.78   &69.19\\  \hline
         \multirow{1}{*}{XLNet}  &85.2   &88.56  &50     &71.10 & 72.31  &51.08   &69.18\\\hline
    \end{tabular}
    }
    \caption{Evaluating consistency and semantic sensitivity of baseline LMs (BERT, ALBERT, and XLNet}
    \label{tab:extra_evaluation}
\end{table*}

\paragraph{Baseline LMs on \auto{}:} In a different set of experiments, we investigate whether \dataset{} is generally challenging to be solved (see Table \ref{tab:evaluation}). Thus, we use three different language models BERT~\cite{devlin-etal-2019-bert}, ALBERT~\cite{lan2019albert}, and XLNet~\cite{yang2019xlnet} in the same architecture described in Sec. \ref{Sec:Architecture} and evaluate their performance on two automatically generated evaluation sets, seen and unseen sets, plus the \human{} test set. To evaluate the models performance on the human test set, we further fine-tune models on \human{} training samples.

We use the unseen test set to check whether the baseline models are using shortcuts in the language surface. This set does not influence the reasoning steps and applies minor modifications in the vocabulary of the stories. The modifications are randomly applied on a number of generated stories and questions to change the names of shapes, colors, sizes, and relationships~(more details in Appendix~\ref{sec:additional_eval}).

All models perform worst in ``YN'' \qtype, which presents a more complicated phenomena due to using quantifiers in the questions. The XLNet model performs best on all \qtype{}s, except the Human evaluation on YN \qtype. However, the drop in the unseen and human test evaluation shows that the model is fitted on the training vocabulary and cannot generalize well. The low accuracy on human test set shows that solving this benchmark is still an open problem and requires more sophisticated methods.

The human performance is evaluated on 100 random questions from \auto{} and \human{} test sets. The respondents are graduate students that were trained by some samples of the dataset before answering the final questions.



% \subsection{Results}
% \rk{YN f1 measure in another table?}\\
% \rk{incomplete}
% \rk{Consistency and contrast part}\\
% \outline{ EXP1-5, selective masking model, test on bAbI and boolQ} \outline{remove 8K results and just mention them as an experiment}\\
% In this section, we compare the results of the experiments introduced in Section~\ref{Sec:Setup}. 

% \pk{this paragraph needs revision, currently it is just confusing, why you bring the calculation here? you even do not mention the results. You can shortly say that "we have done these two tests [cite the reference]" these are harder tests that not only test the correctness but also the same questions should get a similar answer ... [short description of consistency and contrast go here]. The results show lower performance when considering these two metrics which means the LMs remember the language surface and do not necessarily perform an actual spatial reasoning. [Remove 84*80... } 
To evaluate the reliability of the models, we provide two extra consistency and contrast test sets. 
\textbf{Consistency set} is made by changing a part of the question in a way that seeks for the same information~\cite{hudson2019gqa, suhr2018corpus}. Given a pivot question and answer of a specific consistency set, answering other questions in the set does not need extra reasoning over the story.
\textbf{Contrast set} is made by minimal modification in a question to change its answer~\cite{gardner2020evaluating}~(see Appendix ~\ref{sec:cons}).  For contrast sets,  there is a need to go back to the story to find the new answer for the question's minor variations. 
\qn{I don't understand this}\rk{it means that to solve them we should reason over new information from data. not the same infromation taht we used in questions.} The consistency and contrast sets are evaluated only on the correctly predicted questions to check if the actual understanding and reasoning occurs.
This ensures the reliability of the models. %whether the model is reliable on detecting the objects and reasoning about the relations when answering those questions.

Table~\ref{tab:extra_evaluation} shows the result of this evaluation on four \qtype{}s of \auto{}. This table shows that the high result on the seen test set is mainly due to overfitting on training data rather than correct detection of spatial terms and reasoning over them. 


% \pk{both sets together? ore once for consistency and once for contrast? rephrase if it is the second case. }



    
% \outline{on other target tasks}
\paragraph{BERT$_{QA}$--{\small\auto{}} on other dataset} In this experiment, we want to check whether the knowledge learned from \auto{} is transferable to other target tasks or benchmarks. We use BERT$_{QA}$--{\small\auto{}} trained on YN \qtype{} and check its performance on two different benchmarks, bAbI and boolQ, by fine-tuning on their training set.
% These experiments use the trained model on the YN \qtype{} and further fine-tune it on bAbI and boolQ.
% We set two other experiments to check how we can transfer the learning from \auto{} to solve other datasets' problem.


\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/babi_result.png}
    \caption{Results of  BERT and Fine-tuned BERT on \auto{} on different portion of training set of bAbI.}
    \label{fig:babi_train}
\end{figure}
% boolq
\begin{table}[h]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{|l|c|}
        \hline
        \textbf{Model} &\textbf{Accuracy}\\ %\cline{3-14} 
        \hline
          Majority baseline*         & 62.2 \\\hline
          Recurrent model (ReM)*        & 62.2 \\\hline
          ReM fine-tuned on SQuAD*  & 69.8 \\\hline
           BERT (our setup)  & 71.89 \\\hline
          ReM fine-tuned on QNLI*   & 71.4 \\\hline
          ReM fine-tuned on NQ * & 72.8 \\\hline
          BERT fine-tuned on \auto{} & \textbf{74.18} \\\hline
    \end{tabular}
     }
    \caption{Result of fine-tuned version of Recurrent Model and BERT on different dataset. All these results are on the DEV set of boolQ since the test set is not provided yet. *: All models and results are from \cite{clark2019boolq}.} 
    \label{tab:boolq}
\end{table}


Figure \ref{fig:babi_train} compares the performance of BERT and BERT$_{QA}$-{\small\auto{}} on different portions of bAbI training set. Figure \ref{fig:babi_train} shows that BERT$_{QA}$-{\small\auto{}} performs better than BERT when reducing the number of bAbI training samples to 1k, 500, and 100. With 5k and 10k training examples, %samples, 
both models can achieve 100\% accuracy while fine-tuned BERT on \auto{} achieves this performance requiring fewer training epochs (BERT$_{QA}$-{\small\auto{}} achieves 100\% accuracy with 10k training samples, after two epochs while BERT achieves this performance after 6 epochs). In conclusion, using \auto{} reduces the need of large training data and helps models converge quicker.
% \pk{clarify the point of this graph in one clear sentence, something like: Using SPRATQ no need to train on babi to solve the babi task or "Using spartqa smaller number of babi training examples are needed for solving babi task and the models converges quicker" ...}


Table \ref{tab:boolq} shows that fine-tuning BERT on our dataset yields a better result than fine-tuning Recurrent model on SQuAD dataset~\cite{rajpurkar2016squad}, Natural Question dataset NQ~\cite{kwiatkowski2019natural}, and QNLI task from GLUE~\cite{wang2018glue}.
This result is significant since these datasets and tasks are more related to boolQ than \dataset{}. 

% Both boolQ and SQuAD are on the same source data (Wikipedia articles), boolQ builds upon the NQ which contains some natural yes/no questions, and in QNLI task the model must determines if a SQuAD sentence contains the answer to the question or not. 

% Table \ref{tab:boolq} shows that fine-tuning BERT on our dataset yields a better result than fine-tuning Recurrent model on SQuAD dataset (that both boolQ and SQuAD~\cite{rajpurkar2016squad} are from the same source data, Wikipedia articles), Natural Question dataset , NQ~\cite{kwiatkowski2019natural} (that boolQ is built upon this) and QNLI task from GLUE~\cite{wang2018glue} (that determine if a SQuAD sentence contains the answer to the question) on the boolQ benchmark. 
% \pk{i tried to clean this paragraph, but still is grammatical, please revise. what is the "on the boolQ benchmark" at the end!}

Many of the examples answered correctly on boolQ with the fine-tuned BERT on \auto{} required multi-step reasoning. Our hypothesis is that since solving \auto{} questions needs multi-step reasoning, fine-tuning BERT on \auto{} generally improves this capability of the base model.



All experiments, use the models defined in Sec. \ref{Sec:Architecture}. We use AdamW~\cite{loshchilov2017decoupled} with $2\times 10^{-6}$ learning rate and Focal Loss~\cite{lin2017focal} with $\gamma = 2$ for training all the models.

% Regarding question number 3, we provide extra evaluations on the contrast and the consistency sets which show the low performance of the models on some tasks in reasoning over the underlying meaning of spatial relations. This experiment shows the importance of designing such evaluation sets compared to classic seen/unseen test sets.

% Each question in the test set has multiple contrast and consistency questions when possible~(for some questions, it is not possible to generate a complementary set). Answering the consistency questions around a pivot question is possible for human without the need for extra reasoning over the story and based on the main questions' answer. To evaluate the models on these complementary sets, we consider an output to be correct if the main question and its complementary(consistency or contrast) set are answered correctly~(the evaluations of consistency and contrast set are done separately). 
% \pk{both sets together? ore once for consistency and once for contrast? rephrase if it is the second case. }
% The consistency and contrast set evaluations are applied only on the subset of the test set questions answered correctly by the model. This measures the actual understanding of the model when it answers a question correctly. For instance, if a model accuracy is $84\%$ and the consistency result is $80\%$, we can assume that the actual accuracy of the model is $0.84 * 0.80 = 0.672$ on the seen test set.
% We only compute the consistency results on the best performing model on each task. The results of these experiments are shown in Table~\ref{tab:extra_evaluation}.

% \begin{table*}[]
%     \centering
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{|l|c|cc|cc|cc|}
%         \hline
%         \multirow{2}{*}{Models} &  \multicolumn{1}{c}{FB}  & \multicolumn{2}{c}{FR} & \multicolumn{2}{c}{CO} & \multicolumn{2}{c|}{YN}\\ \cline{2-8}
%          &Consistency&Consistency&Contrast&Consistency& Contrast&Consistency& Contrast\\ \hline
%          \multirow{1}{*}{BERT}&81.43&86.07&60.06&74.06&92.45&33.89&39.26\\ \hline
%          \multirow{1}{*}{AlBERT} &82.50&93.28&76.83&11.50&50.50&32.39&30.46\\  \hline
%          \multirow{1}{*}{XLNet}& 83.92& 93.49 &79.76& 89.02 & 97.04 & 39.17 & 48.33\\\hline
%     \end{tabular}
%     }
%     \caption{Consistency and Semantic Sensitivity of Models}
%     \label{tab:extra_evaluation}
% \end{table*}

% We compare the complexity of our generated stories and questions with the bAbI task 17. As bAbI questions have Yes/No answers, we apply the same model of our ``YN'' task to bAbI. The BERT model on the test set of the small variation of bAbI (training examples) yields $99.9\%$ accuracy. This indicates the simplicity of the bAbI dataset comparing to our newly generated stories and questions of the same type. 
% In the end, we have evaluated the fluency and complexity of our generated stories with the human-generated stories. This experiment is done by providing a mixture of human-generated stories and \dataset{} stories to participants and ask them to tag the author of the passage with either a human or a machine. We have made a random list of 8 human-generated stories~(from 3 authors on the same data) and eight generated stories of the dataset and arranged them randomly in a sequence. Each participant receives the sequence one by one and tags them with an appropriate author. No feedback is provided to the participants during the test. 
% The result of this experiment shows that our stories are wrongly tagged as human-generated in $57.5\%$, and the human-generated stories are wrongly tagged as machine-generated in $47.5\%$ of the responses. These results indicate an almost total uncertainty in detecting the author of the stories, which provide evidence of the high resemblance of our stories to what a human has made on the same data. Thus, the quality of the proposed stories are comparable to human-generated stories and can reflect the same level of difficulty. The code, data, and all related material will be publicly available.


% \subsection{pretraining and fine-tuning}
% In order to make BERT compatible with our QA as the downstream task, we train BERT on a subset of our generated data. We evaluate two versions of BERT pretrained and fine-tuned on our data to evaluate its understanding of spatial reasoning against the human-generated set. 

% First, we get the pretrained BERT and fine-tune it further on a subset $D_{1}$ with size 500 stories from our training set. Then, we evaluate BERT performance fine-tuned on $D_{1}$ on the human-generated stories to get the performance of BERT on spatial reasoning.

% Second, we first further pretrain BERT on masking some parts of our selected stories and then fine-tune it on the final task of QA. The evaluation process is the same as described in first scenario.

% \subsection{Heavy supervision baselines}
% \label{supervision}
% \outline{The baseline which already solve the bAbI 20task dataset, and its result on this ones.}\\
% \outline{More complex model for finding the annotations.}

